Multi-Step Adversarial Perturbations on Recommender Systems Embeddings

Recommender systems (RSs) have attained exceptional performance in learning users' preferences and helping them in finding the most suitable products. Recent advances in adversarial machine learning (AML) in the computer vision domain have raised interests in the security of state-of-the-art model-based recommenders. Recently, worrying deterioration of recommendation accuracy has been acknowledged on several state-of-the-art model-based recommenders (e.g., BPR-MF) when machine-learned adversarial perturbations contaminate model parameters. However, while the single-step fast gradient sign method (FGSM) is the most explored perturbation strategy, multi-step (iterative) perturbation strategies, that demonstrated higher efficacy in the computer vision domain, have been highly under-researched in recommendation tasks. In this work, inspired by the basic iterative method (BIM) and the projected gradient descent (PGD) strategies proposed in the CV domain, we adapt the multi-step strategies for the item recommendation task to study the possible weaknesses of embedding-based recommender models under minimal adversarial perturbations. Letting the magnitude of the perturbation be fixed, we illustrate the highest efficacy of the multi-step perturbation compared to the single-step one with extensive empirical evaluation on two widely adopted recommender datasets. Furthermore, we study the impact of structural dataset characteristics, i.e., sparsity, density, and size, on the performance degradation issued by presented perturbations to support RS designer in interpreting recommendation performance variation due to minimal variations of model parameters. Our implementation and datasets are available at https://anonymous.4open.science/r/9f27f909-93d5-4016-b01c-8976b8c14bc5/.

==> Backup/4Discussion.tex <==
In this section, we discuss the experimental results to answer the previously defined open questions on the effectiveness of iterative attacks, the impact of structural dataset characteristics on the robustness of the model under attack, and the fairness variation of the perturbed RSs.

\subsection{RQ1. Investigating the effect of iterative attacks against the recommender performance accuracy.}

\input{images/figures}
This study aims to measure the effects of adversarial attacks on accuracy and beyond-accuracy objectives. In particular, to better understand the merits of the presented adversarial attacks, we aim to answer the following evaluation questions:

\begin{itemize}
    \item \textbf{On the attack side}: how much adversarial perturbations obtained from the single-step FGSM and the two iterative BIM and PGD attack methods can impair the quality of the original BPR-MF model? The answer to this question can be found in Fig.~\ref{fig:a} \&  Fig.~\ref{fig:c} by comparing the original non-attacked model with the rest.

    \item \textbf{On the defensive side}: what is the impact of adversarial training on BPR-MF using the state-of-the-art AMF recommender model on the previous question?
    % Does the adversarial training mod impact iterative attacks more/less than single-step attacks? 
    The answer to this question can be found in Fig.~\ref{fig:b} \& Fig.~\ref{fig:d}.
    
\end{itemize}

% to compare the performance of the original non-attacked recommenders (e.g., xxx, xxx \yashar{random, BPR-MF?}) with the attacked ones, i.e., BMPR-MF model parameters are perturbed by the FGSM, BIM, and PGD attacks and (ii) to compare the impact of defensive AMF 

In this line, since the performance of the two presented of multi-step adversarial attacks varies based on the number of iterations in Section~\ref{subsubsec:impact-iterations}, we discuss and analyze the effectiveness of the presented attacks across different
iterations. Afterward, in Section~\ref{subsubsec:impact-epsilon}, we relax the iteration dimension, and for a fixed iteration number, we study how adversarial perturbation budget $\epsilon$ impairs recommendation outcome.

% To assess the effect of multi-step attacks comparing to the single-step attack  we compare three different level of investigation on accuracy, and beyond accuracy, performance.
% \alejandro{I think this sentence should be rewritten: compare appears twice, 'three different level' is incoherent and redundant (it is obvious that you will not use two levels which are the same), and 'level of investigation' it is not clear to me what you mean with it}~\felice{I have rewritten it.}
%To study iterative attacks we explore their effect on accuracy and beyond accuracy metrics changing the number of perturbation and the $\epsilon$-limited budget perturbation. 


\subsubsection{Impact of iterative attacks based on number of iterations.}~\label{subsubsec:impact-iterations}
% \updated{Fig.~\ref{fig:overall_effect} visualizes the performance (accuracy and beyond-accuracy) variations by increasing the number of iterations for the \lfm dataset. We rely on a plot visualization only for the \lfm dataset to clarify the insights obtained vividly. We show the performance of random recommender to serve as a lower baseline. Table~\ref{table:auc} however, summarizes the complete results obtained across various evaluation measures and recommendation/attack models on both the \ml and \lfm datasets. Please note that given the large set of evaluation metrics chosen, for the space limitation, in Table~\ref{table:auc} we report the normalized accumulated values of the performance across iterations for all the experimented cases.}
Fig.~\ref{fig:overall_effect} visualizes the performance (accuracy and beyond-accuracy) variations by increasing the number of iterations for the \lfm dataset. We rely on a plot visualization only for the \lfm dataset to vividly display the obtained insights. We show the performance of random recommender to serve as a lower baseline. 
Then, Table~\ref{table:auc} summarizes the complete results obtained across various evaluation measures and recommendation/attack models on both the \ml and \lfm datasets. 
For space limitation, Table~\ref{table:auc} reports the normalized accumulated values of the measured recommendation performance across iterations for all the experimented cases due to the large set of examined metrics.


%overview of the accumulated normalized values of accuracy and beyond accuracy metrics evaluated on both the \ml and \lfm datasets to compare the initial not-attacked recommender with the attacked ones, i.e.,  recommenders perturbed by the FGSM, BIM, and PGD attacks.

%variation of accuracy performance with respect to increase in number of interactions at varying the number of attack iterations on the \lfm dataset for a matter of space.While Figure~\ref{fig:overall_effect} is a visual snap-shot of accuracy results for the \lfm dataset,  Table~\ref{table:auc} reports a complete overview of the accumulated normalized values of accuracy and beyond accuracy metrics evaluated on both the \ml and \lfm datasets to compare the initial not-attacked recommender with the attacked ones, i.e.,  recommenders perturbed by the FGSM, BIM, and PGD attacks.}
On the attack side, by looking at Fig~\ref{fig:a} one can note that both multi-step attacks, i.e., BIM and PGD, are more powerful compared with the state-of-the-art single-step FGSM attack, for a fixed perturbation budget $\epsilon=0.5$. We can realize that only after 25 iterations, the $nDCG$ of PGD drops from the original 0.2033 to 0.0080, which is much lower than FSGM (0.12155). For instance, the PGD attack shows \textbf{15.1} (0.12155 v.s. 0.00804), \textbf{20.4} (0.12155 v.s. 0.00595), and \textbf{23.8} (0.12155 v.s. 0.00510) times stronger impact with respect to FSGM, for 25, 40, and 50 iterations respectively. 
These results confirm the findings in the CV field~\cite{DBLP:conf/iclr/KurakinGB17a} on the superiority of iterative adversarial strategies --- in terms of attacks' effectiveness --- compared to single-step ones for the item recommendation task. They also demonstrate the vulnerability of the de-facto pairwise ranking model (BPR-MF) against modern adversarial perturbations. To better understand the fragility of defense-free BPR against iterative attacks, we have also shown the performance of the random recommender.  And in fact, the victim BPR-MF model starts to act like a random recommender in terms of recommendation accuracy only after iteration 25, i.e., the model almost loses all information it had learned about the preference of individual users.

%\yashar{@Felice: here you could you say sth briefly about beyond-accuracy?Icov. I would mention that interestingly it has a varying behavior based on iterations and can be perhaps set by the system designer. I am going to rely on it when explainaing the Table.}\\

%making completely vain all the learning effort

%CV results on the superior power of iterative adversarial strategies compared to single-step ones and demonstrate the weakness of the experimented model-based recommenders against small perturbations of the parameters.

% \yashar{These results are interesting and show (say sth here, we can say they confirm what was reported in CV but the impact seems to be lower since metrics/task everything is different)}

%(0.00804 v.s. 0.20333) , The effectiveness of the PGD attack with respect to FGSM at iterations 25, 40 and 50 is as follows: 25.2 (0.00804 v.s. 0.20333) ,  }

%\updated{Both multi-step attacks were very successful when compared to the state-of-the-art FGSM-like approach with a fixed perturbation, i.e., $\epsilon=0.5$. For instance, Figure~\ref{fig:a} shows an extreme worsening of accuracy performance (i.e., $nDCG$) on the \lfm dataset such that the victim recommender starts to behave like a random recommender after about 25 iterations ($L=25$) making completely vain all the learning effort. For instance, $nDCG$ remains stable between 0.08 and 0.12 when iterative attacks computes more than 25 iterations (see Figures~\ref{fig:a} and~\ref{fig:b}). 


The same pattern of results can be noticed by looking at the overall results shown in Table~\ref{table:auc}, where for all <dataset, recommender> combinations, the iterative attack strategies (PGD and BIM) outperform FSGM. For instance, the <\ml, BPR-MF> combination shows that the accuracy performance under the PGD attack is reduced by more than 2 times compared to FGSM, e.g., (0.0074 v.s. 0.0035), (0.0740 v.s. 0.0353), and (0.0368 v.s. 0.0172) for $PR$, $RE$, and $nDCG$ respectively.

%\updated{The same difference is around 10 times for the \lfm dataset}. \yashar{should we say this too?}~\felice{I think we have said a lot for lfm already}\yashar{yeah sure ok let's go forward an dtry to complte this part}
% \yashar{explain a few more sentences more, or give an example}ok
\input{tables/AUC-ml1m}

Here, we should point out that both Figure~\ref{fig:overall_effect} and Table~\ref{table:auc} do not show a clear difference/advantages of PGD attack compared to BIM attack. This finding is different from the one previously reported by Athalye \textit{et al.}~\cite{DBLP:conf/icml/AthalyeC018} in CV. We motivate it by the fact that the item recommendation model BPR is less sensitive to the initial value of weights compared with a classification task by using a deep neural network, since in BPR the gradients are computed based on the differences between pairs. 

%\yashar{If it was shown in CV why do we say BPR is different?}~\felice{Because results show that PGD and BIm behaves almost similarly in the case of BPR-MF, while in CV PGD is better than BIM} \yashar{in that case, we should update this sentence his finding was previously reported by Athalye \textit{et al.}~\cite{DBLP:conf/icml/AthalyeC018} in CV.}~\felice{There is already the citation to that paper}

For what concerns beyond-accuracy analysis, we found an interesting behavior for the defense-free BPR-MF. We can see that during the first 25 iterations of BIM, $ICov$ increments nearly by 76\% (from 6220 to 10928) compared to the coverage value of the not-attacked recommender (see Fig.~\ref{fig:c}). After that, it steadily diminishes with a minimum $ICov$ value of 1948 (for BIM).
This result may be justified by the fact that when the multi-step attack is very destructive on the accuracy measures, then the model will start to recommend a set of few items all the users will not appreciate. Regardless of this, for all iterations, the performance is considerably lower than the random recommender. Interestingly, we can assert that the proposed iterative attacks impair the personalized recommender to perform as bad as as a random recommender (see Fig.~\ref{fig:a}) concerning accuracy measure and even worse with respect to beyond-accuracy measure. As an example of the latter, consider $ICov$ is 19105 in Random, and 1948 for BPR-MF attacked by BIM with 260 iterations, a difference of about 90\% . Note that, Table~\ref{table:auc} confirms very low beyond-accuracy metric values also for $EFD$ and the $SE$. The iterative attacks reduced both metrics by more than $50\%$ and $20\%$ respectively independently from the <dataset, recommender> combination.

%in a state where the accuracy performances are very bad as a random recommender (see Fig.~\ref{fig:a}), and the beyond-accuracy measures are even 90\% smaller than the ones of the random model, e.g., $ICov$ is 19105 in Random, and 1948 for BPR-MF attacked by BIM with 260 iterations. It follows that \textit{the iterative perturbed model behaves even worse than a random model}.

% yashar{here we can say in terms of beyond-accuracy the attacked model works better than random recommender.}


%looking at the training of deep neural network classifiers which are directly influenced by the weight initialization. For instance, an initializing weight to zero (as in BIM) the classifier will be completely different from a random weight initialization (as in PGD). While BPR is more robust to the initial value of weights because the gradients are computed on the difference between pairs.

%These results are also confirmed by the overall results shown in Table~\ref{table:auc}. In fact, all <dataset, recommender> combinations got the best attack effectiveness in the case of iterative strategies. However, both Figure~\ref{fig:overall_effect} and Table~\ref{table:auc} do not show a clear improvement of PGD attacks compared to BIM attacks, as recognized by Athalye \textit{et al.} ~\cite{DBLP:conf/icml/AthalyeC018} in the computer vision domain. For instance, Table~\ref{table:auc} does not show a clear pattern on which is the most powerful iterative attack version. ~\felice{We motivate this finding looking at the training of deep neural network classifiers which are directly influenced by the weight initialization. For instance, an initializing weight to zero (as in BIM) the classifier will be completely different from a random weight initialization (as in PGD). While BPR is more robust to the initial value of weights because the gradients are computed on the difference between pairs.} \alejandro{any comment about how or why BIM and PGD are so close to each other?}
% \alejandro{any reason for this? will this be answered or discussed later? if so, I would point to that here}
% \yashar{I would suggest to explain more about AMF than beyond-accuracy which follows this paragraph.}\\
On the defensive side, we studied the impact of adversarial training, known as AMF, on various attacks' performances. We observed an evident decrease in accuracy performance in AMF (see Figure~\ref{fig:b}), which is, on average, more than 58\% for multi-step strategies and 11.31\% for the single-step one (see Table~\ref{table:auc}). For instance, the PGD attack shows \textbf{1.48} (0.21471 v.s. 0.14483), \textbf{1.86} (0.21471 v.s. 0.11541), and \textbf{1.94} (0.21471 v.s.  0.11060) times stronger impact with respect to FSGM, for 20, 30, and 50 iterations respectively. 

% \yashar{could you please add the raw values here? since when we say decrease it is not clear if we are looking from value perspective or attacker perspective.} 

% However, iterative attacks have caused an average performance decrease of more than 98\% on BPR-MF.\\

%Then, we compared the different effects of iterative attacks applied against the not-defended model, i.e., BPR-MF, and the adversarial protected one, i.e., AMF. We observed an evident decrease in accuracy performance in AMF (see Figure~\ref{fig:b}), which is, on average, more than 58\% for multi-step strategies and 11.31\% for the single-step one (see Table~\ref{table:auc}). However, iterative attacks have caused an average performance decrease of more than 98\% on BPR-MF. Such considerations reveal that \textit{iterative attacks are more effective than FGSM-like also in defense settings, but the adversarial training has reduced the destructive impact of our proposed attacks, and it has protected the victim recommender avoiding the production of quite random recommendation lists.}


% \alejandro{Table 2 has already been mentioned a couple of times, I miss a comment or note in the text about the nature of the values presented in the table, that is, that those are not standard values but AUC, or accumulated normalized values of the metrics across the iterations}

% \yashar{the following should be reduced}
% Motivated by intriguing effectiveness of iterative attacks in drastically reducing the recommender model accuracy, we explored beyond-accuracy metrics. 
% % \alejandro{why misusing? what do you mean? why do you say this?}~\felice{I used misusing to say that the accuracy became b}
% Table~\ref{table:auc} shows a clear worsening of the novelty and diversity metrics evaluated on adversarially altered recommenders. For instance, the $EFD$ goes down more than $50\%$ independently from the dataset and recommender. The deterioration of recommendation performance is shown also on the other beyond accuracy measures. In fact, getting the expected free discovery $EFD$ to smaller values, reducing the Shannon Entropy $SE$ by more than the $20\%$, and dropping the $ICov$ by more than 50\%, Table~\ref{table:auc} clearly shows that the proposed multi-step attack strategies can effectively break also the ability of a recommender model to suggest diverse and long-tail products. We justify this result by the fact that an iterative attack is strongly optimized to corrupt the knowledge of user's preferences---- the adversary maximizes the model loss function--- leading the perturbed recommender to not able to generate well-personalized recommendations.\yashar{till here}


% \alejandro{In this paragraph I would remove the '@10' from the metrics.}

% \alejandro{In the table, I would add a comment about what bold means, since usually it represents the best (highest) results, so it might be very confusing realising that it represents the opposite (in this paper it makes sense, but I would emphasise that in the caption)}



%\alejandro{I think the results in the figures could be discussed in more detail. Like: what is importance of the point where a recommender starts behaving like a random predictor?}~\felice{After the iteration 25 it starts to get almost random performance. I have added this value in the discussion.}

%\alejandro{what about the better performance in AMF? what about the drop in coverage? I think today you mentioned something about this and linked it to popularity bias} ~\felice{I have added}


%\alejandro{Are these results similar for ML (even though for the sake of space they are not shown here)?}~\felice{Yes, they are the same. I have better explained that we put teh figure only for Last FM for  a matter of space but we have inserted the AUC results for all datasets and recommenders in the Table2.}



\subsubsection{Impact of iterative attacks based on $\epsilon$-limited budget perturbation.}~\label{subsubsec:impact-epsilon}
\input{images/figures-eps}
In this study, we release the investigation of the impact of iteration increase on iterative attacks' performances. Instead, by fixing the number of iterations (i.e., $L=25$) and varying $\epsilon$ from $0.001$ to $10$, we investigate at what  $\epsilon$-level, iterative attacks can get a similar performance comparable with FGSM. We found that iterative adversarial strategies reach the FGSM performance for $\epsilon=0.5$ at iteration-level $\epsilon \simeq 0.1$. In other words, by using $\frac{0.5}{0.1}=$\textbf{5} timeless perturbation budget, the presented iterative strategies reach a similar performance as that of the state-of-the-art attack strategy.


%After having tested the efficacy of multi-step adversarial perturbation compared to single-step ones, the budget perturbation $\epsilon$ is fixed (i.e., $\epsilon=0.5$ in Figure~\ref{fig:overall_effect}), we investigate the possibility to get FGSM-similar performance with even a smaller perturbation of model parameters. For instance, Figures~\ref{fig:eps-a} and~\ref{fig:eps-b} report the result of performing BIM and PGD, attacks by fixing the number of iterations (i.e., $L=25$), and varying $\epsilon$ from $0.001$ to $5$. We uncover that iterative adversarial strategies reach the FGSM-performance with $\epsilon<0.5$ (e.g., BIM attack in Figure~\ref{fig:eps-a} surpasses FGSM with $\epsilon \simeq 0.01$).  Here, we draw the following consideration: \textit{iterative adversarial strategies can generate a worsening of recommendation performance comparable to FGSM attack with even a smaller perturbation budget ($\epsilon$)}.

\yashar{I have transferred the summary here}
\updated{\textit{In summary, the results of two above studies provides strong evidence that iterative attacks presented for item recommendation task in this work are much more stronger than single-step version (FGSM attack model) used widely in prior literature. For instance, for a fixed perturbation budget $\epsilon = 0.5$, with only 25 iterations, the new attack strategies weaken the not-defended BPR-MF performance by an amount of 15 times (along $nDCG$). We also showed an equivalent comparison between these attack strategies contemplating the fact that iterative attacks can reach similar performance of FSGM by using only 2\% of the perturbation budget $\epsilon$.}}\yashar{will need to say about defended model too}

%Let us summarize the previous observations: \textit{given a fixed perturbation budget ($\epsilon$), iterative attacks are much more powerful than single-step versions both in leading low-accuracy recommendation performance, even similar to one of the random recommenders and in making even more difficult the addressing of the recommendation problem to produce a diverse and novel recommendation. However, we do not find e considerable improvement of PGD with respect to BIM as demonstrated in adversarial attacks to fail the image classification tasks.}.
\subsection{RQ2. Studying the impact structural dataset characteristics on the efficacy of adversarial attacks.}
\input{images/figure-sparsity}

% \alejandro{URM was never defined before}

The second part of our investigation relates to the effect of structural dataset characteristics on the efficacy of adversarial attacks. 
Inspired by the exploratory study on impact of dataset characteristics on shilling attack efficacy proposed in~\cite{sisinflabSigir2020}, we evaluated the impact of the \textit{density}, \textit{size}, and \textit{shape} structural features in the variation of an accuracy metric ($nDCG$) under adversarial perturbation on the model parameters, defined $ \nicefrac{|\mathcal{F}|}{|\mathcal{U}| \times |\mathcal{I}|}$, $|\mathcal{U}| \times |\mathcal{I}|$, and $\nicefrac{|\mathcal{U}|}{|\mathcal{I}|}$ respectively. 
We produced 10 sub-samples for each dataset with different levels of structural features. Each sub-sample is a \textit{k-core} version of the original datasets, such that we removed users and items with lesser than \textit{k} recorded interactions.
Note that increasing the \textit{k} from 10 to 100, we were able to generate sub-samples with increasing \textit{density}. 
% \alejandro{I've been asked several times to define what a k-core is, I would briefly define it here}


Figure~\ref{fig:sparsity} shows the percentage change of the accuracy measure, i.e., $\Delta nDCG$, evaluated before and after the adversarial perturbation. In line with what has been shown in~\cite{sisinflabSigir2020} on the impact of dataset characteristics on the effectiveness of hand-engineered shilling attacks against collaborative recommenders, results in Figure~\ref{fig:sparsity-a}, and~\ref{fig:sparsity-d}, confirm that increasing the \textit{density} of the dataset an attack is less effective ---$\Delta nDCG$ is smaller----.
Furthermore, we continue the investigation exploring the impact of the \textit{size} and the \textit{shape} characteristics. 
We report in Figure~\ref{fig:size-b}, \ref{fig:shape-c}, \ref{fig:size-e}, and~\ref{fig:shape-f} the $\Delta nDCG$ results at varying of the \textit{size} and \textit{shape} characteristics. We uncovered that the \textit{size} and \textit{shape} shown a similar visual trend-- the $nDCG$ increases when the shape/size increased---. Interestingly, also \textit{size} and \textit{shape} influences on the effect of adversarial attacks are consistent with the one described with an explanatory models in shilling attack analysis in~\cite{sisinflabSigir2020} on model-based recommenders (i.e., MF).

Let us summarize previous findings: \textit{structural dataset characteristics (i.e., shape, space, and density) have a decisive influence on the effectiveness of adversarial attacks against model-based CF recommenders such that: adversarial perturbations are less impactful by either increasing the density or decreasing the shape or the size}.


\input{tables/results_fair}
\subsection{RQ3. Fairness Evaluation.}
In this section, we analyze the impact of attacking a recommender system, i.e., BPR-MF, under a fairness perspective.
Fairness analysis is becoming increasingly important in the last years in several machine learning-related fields.
As a matter of fact, recommendation algorithms are prone to generate algorithmic biases, reproduce biases in data, or to inherit prejudices in training data~\cite{DBLP:journals/ir/BelloginCC17,DBLP:conf/cikm/ZhuHC18,DBLP:conf/recsys/DeldjooAZKN19}.
In this scenario, analyzing fairness is important than ever, since a substantial variation of recommendation performance for the different groups of users, or categories of items, may unveil the attacker.
To this purpose, we have measured the accuracy performance considering the different groups/categories, and three fairness metrics, namely GCE, MADr, and MADR, exploring both the initial and attacked models, to capture the original behavior and contrast it against the observed one after the attacks.
In detail, GCE considers several possible ideal probability distributions for each user, or item, clustering. 
Hence, it computes the divergence of the recommendation results (by considering a specific metric, i.e., nDCG) from the ideal distributions.
Consequently, GCE with a value closer to zero denotes the recommender's congruence with that specific probability distribution.
On the other hand, MAD focuses on the absolute variation of a given metric from an ideal situation in which groups/categories are treated equally.
The original formulation of MAD, namely MADr, considers the <user,item>'s scores pairs in the recommendation results.
Additionally, we have also considered a later extension of MAD proposed in~\cite{DBLP:conf/recsys/DeldjooAZKN19}, MADR, in which the per-user performance values of an accuracy metric (i.e., nDCG) are considered. 

Before focusing on fairness, let us analyze the behavior of recommenders for the different groups/categories to uncover the potential biases produced or removed by the attack strategies.
Table~\ref{t:q1} depicts the nDCG performance of the recommenders (BPR-MF, AMF, and their attacked variants) regarding the clusters for three attributes: item popularity, user gender, and user interactions.
The clustering for item popularity and user interactions was computed by considering the quartiles for the attributes, while user gender is naturally clustered in the original datasets.
This table shows, as already noted in the literature, that BPR-MF achieves higher values of nDCG for popular items for both \ml and \lfm. 
In this respect, please note the BPR-MF performance in $C_4$ with the Item pop attribute.
% <Item-Pop,C4> 
% \alejandro{I am not sure this notation <a,b> is easy to follow, was it used before in the paper? In that case it could be used, but this section should not use a different notation as the one used before, so I would say something like 'note performance in $C_4$ with the Item pop attribute'; later on it could be abbreviated, but for the first time, I would not be so cryptic.}
Notably, the efficacy of the attacks is particularly evident here, since, for BPR-MF, the $C_4$ for the Item pop attribute column shows a degradation of the performance when the recommender is under attack.
On the other hand, when the recommender is defended, i.e., AMF, the deterioration of the performance is less evident, even though the trend in the approaches remain the same.
Considering the user gender, we observe that in both datasets the recommendation performance for males ($C_1$) is higher than for women. 
Even though the trends are similar to those observed for item popularity, it is worth noticing that the degradation and the defense effects are more evident in \lfm.
Finally, the table shows two opposite behaviors for user interactions: in \ml, BPR-MF seems to favor the less active users, whereas \lfm favors the most active ones.
This is probably due to the different number of items in the catalog together with the well-known strong popularity bias present in \ml; moreover, cold users in this dataset include more information than in \lfm, so those categories are not completely comparable. \alejandro{Walter, could we mention here the number of interactions that separate C1 from C2 in each dataset?}
, that provides good information for cold user profiles. 
It is an interesting aspect that, in another context, deserves a specific study.
\alejandro{If what I added is true, I would remove the previous sentence}
\input{tables/stat-gorups}
% ok, now we analyse the performance for the attack strategies...
Regarding the change in performance when using any of the attack methods, we observe that in \ml the trend and absolute values remain almost the same with respect to the initial recommender; however, in \lfm the situation is not identical: while the degradation follows the same trend, defended methods (AMF) show higher accuracy values for all the clusters.
% \alejandro{if there is nothing else to discuss about this, then I would join this part with the previous paragraph}

\alejandro{one problem with the previous analysis is that, since we are only discussing performance, it might not be seen as 'fairness analysis', I tried to make this clear at the beginning that this helps on understanding fairness, but would like to know what you (Walter, Yashar) think}\walter{I completely agree with you, but I think that the analysis we provided at the beginning is interesting. Maybe we can also change the title of the section to be on the safe side.. What do you think?}\yashar{I think both studies share similarity in the sense that we get fine-grained insights per group/cluster. However GCE doesn't care about the actual values, it shows deviation from distribution without giving us intuition at what performance this was achieved. Table 3, looks like "per-class" performance evaluation. What about calling this section sth along: "Per-class validation and fairness"?}

%% now we discuss results about fairness metrics
%\alejandro{the following part is not needed}
%Regarding GCE, we have considered five distinct ideal probability distributions, with f0 being the equality based one [0.25,0.25,0.25,0.25], while f1, f2, f3, f4 strongly preferring a specific cluster, [0.7,0.1,0.1,0.1], [0.1,0.7,0.1,0.1], [0.1,0.1,0.7,0.1], [0.1,0.1,0.1,0.7], respectively.
%For User Gender, we have considered three ideal distributions, f0,f1, and f2, being [0.5,0.5], [0.75,0.25], and [0.25,0.75].
Once we have analyzed the performance found in an attribute basis (for some sensitive attributes), we show in Table~\ref{t:q4} the result of the fairness-aware evaluation metrics described before.
We first analyze which of the ideal distributions is better approximated by the initial methods and whether this situation changes when we use a defended model.
%We can analyze the BPR-MF fairness rows. The lowest value per clustering suggests that BPR-MF recommendations follow that cluster distribution.
%Hence, we can understand better the behavior of BPRMF. In detail, we have f1 (<ML,User-gender>), f0 (<ML,User-Interactions>)  f0 (<Last.fm,User-Interaction>).
%We can note that <f0,BPRMF,ML,User-gender> is -0.135 while <f0,AMF,ML,User-gender> is -0.141. It suggests that the defended variant diverges more from that distribution.
%I imagine this analysis per <dataset,clustering>:
%<ML,User-gender>
%The fairness for males is preserved, but the divergence from f0, f2 is higher: AMF is even more "biased/unfair" since it preferers males more than BPR-MF
%<ML,User-Interactions>
%f0 and f4 are lower in AMF. If we focus on f4, this means that AMF is recommending "better" to more active users. This is confirmed by <Table3,ML,User-Interactions,C4,AMF>.
With this goal in mind, we analyze the GCE fairness values corresponding to the initial methods, without and with defense. We observe a consistent behavior in both datasets: the order derived from the GCE values is the same for BPR-MF and AMF. However, for some cases the actual values are different, meaning that the defendent variant diverges in a different way (either more or less) from that distribution than the original method; for instance, for item popularity in \ml, the uniform ($f_0$) and least popular items ($f_1$) obtain a lower absolute GCE value for the defended model, whereas the behavior is the other way around for user interactions in \lfm.
An interesting case is the one of the user gender, where in \ml the divergence for males ($f_1$) is decreased, whereas in \lfm is the opposite; this evidences a non-predictable effect of the defended models with respect to some attributes.
%%
Let us now study whether the defense and/or attack methods modify the fairness performance. 
% performance in clusters are very different, and it tends to be higher under AMF
For this, we observe that some attack methods like BIM help to increase the fairness on some distributions (or attribute values) at the expense of others, such as $f_1$ for user gender and $f_4$ for user interactions in \ml, at the expense of $f_2$ and $f_1$ respectively. %% this happens for BPR-MF and AMF, so it is easier not to say anything else
%%
Finally, we explore whether any attribute is more sensitive under a fairness perspective, since this may be a strong signal that a recommender is under attack.
% attacks are not sensible to fairness when measured for ranking, they are sensible for rating (MADr). This is not completely true for Lastfm.
Thus, we note that FGSM tends to obtain very similar GCE values and MADR values in almost every scenario, whereas MADr tends to change whenever an attack is performed. Because of this, we conclude that if we measure fairness based on ranking performance (i.e., according to GCE or MADR), an FGSM attack might go unnoticed, whereas MADr is more sensitive to any attack. On the other hand, the rest of the attack strategies seem to change too much the distribution of the recommendations, as it becomes evident in the GCE values of item popularity.

\iffalse
\walter{begin raw draft}
\begin{itemize}
    \item What is the nDCG performance of the recommenders considering the different clusters? Does it change if we consider attacks (for the original, and the defended approach)?
    \begin{itemize}
        \item \walter{done}
    \end{itemize}
    \item What is the fairness distribution that approximates best the original BPR-MF?
    \begin{itemize}
        \item We can analyze the BPR-MF fairness rows. The lowest value per clustering suggests that BPR-MF recommendations follow that cluster distribution.
Hence, we can understand better the behavior of BPRMF. In detail, we have f1 (<ML,User-gender>), f0 (<ML,User-Interactions>)  f0 (<Last.fm,User-Interaction>).
    \end{itemize}
    \item Does it change when we defend BPR-MF? Why?
    \begin{itemize}
        \item Now we can analyze what happens when an adversarial defense is applied (AMF).
We can note that <f0,BPRMF,ML,User-gender> is -0.135 while <f0,AMF,ML,User-gender> is -0.141. It suggests that the defended variant diverges more from that distribution.
I imagine this analysis per <dataset,clustering>:
<ML,User-gender>
The fairness for males is preserved, but the divergence from f0, f2 is higher: AMF is even more "biased/unfair" since it preferers males more than BPR-MF
<ML,User-Interactions>
f0 and f4 are lower in AMF. If we focus on f4, this means that AMF is recommending "better" to more active users. This is confirmed by <Table3,ML,User-Interactions,C4,AMF>.
    \end{itemize}
    \item Does the defense and/or the attacks modify fairness performance? How? 
    \begin{itemize}
        \item performance in clusters are very different, and it tends to be higher under AMF
    \end{itemize}
    \item Does any of the clusterings seem to be more affected under the fairness perspective?
    \item Can be the fairness analysis a signal that the recommender is under attack? Or the attack is transparent?
    \begin{itemize}
        \item attacks are not sensible to fairness when measured for ranking, they are sensible for rating (MADr). This is not completely true for Lastfm.
    \end{itemize}
\end{itemize}

\newpage

\fi



==> images/figure-intro.tex <==
% \begin{figure}[t]
%         \centering
%         \begin{subfigure}[b]{0.45\textwidth}   
%             \centering 
%             \includegraphics[width=\textwidth]{images/LastFM/BPR-MF_Recall_Top10.png}
%             \caption[BPRMF]%
%             {{\small $Recall@10$ of BPR-MF on the \lfm dataset}}    
%             \label{fig:intro-plot-a}
%         \end{subfigure}
%         \quad
%         \begin{subfigure}[b]{0.45\textwidth}
%             \centering
%             \includegraphics[width=\textwidth]{images/LastFM/BPR-MF_SE_Top10.png}
%             \caption[BPRMF]%
%             {{\small $SE@10$ of BPR-MF on the \lfm dataset}}
%             \label{fig:intro-plot-b}
%         \end{subfigure}
%         \label{fig:intro-plot}
        
% \end{figure}


==> images/figure-user-groups.tex <==
\begin{figure}[!t]
        \centering
        \begin{subfigure}[b]{0.48\textwidth}   
            \centering 
            \includegraphics[width=\textwidth]{images/LastFM-groups/BPR-MF_nDCG_Top10.png}
            \caption[BPRMF]%
            {{\small BPR-MF}}    
            \label{fig:group-a}
        \end{subfigure}
        \quad
        \begin{subfigure}[b]{0.48\textwidth}
            \centering
            \includegraphics[width=\textwidth]{images/LastFM-groups/AMF_nDCG_Top10.png}            \caption[BPRMF]%
            {{\small AMF}}    
            \label{fig:group-b}
        \end{subfigure}
                \vskip\baselineskip

        \begin{subfigure}[b]{0.48\textwidth}   
            \centering 
            \includegraphics[width=\textwidth]{images/ML1M-groups/BPR-MF_nDCG_Top10.png}
            \caption[BPRMF]%
            {{\small BPR-MF}}    
            \label{fig:group-a}
        \end{subfigure}
        \quad
        \begin{subfigure}[b]{0.48\textwidth}
            \centering
            \includegraphics[width=\textwidth]{images/ML1M-groups/AMF_nDCG_Top10.png}            \caption[BPRMF]%
            {{\small AMF}}    
            \label{fig:group-b}
        \end{subfigure}
        \caption[AMF]
    {\small Last FM results with Iterative Attacks at varying of users' groups. The bars are the average number of rating in each group.} 
    \label{fig:group}
    
\end{figure}

==> images/test-figures.tex <==

\begin{figure}[!th]

        \centering
        \begin{adjustbox}{minipage=\linewidth,scale=1.2}
        \begin{subfigure}[b]{0.24\textwidth}
            \centering
            \includegraphics[width=\textwidth]{images/LastFM/BPR-MF_nDCG_Top10.png}
            \caption{\small  \textbf{BPR-MF}}
            \label{fig:testa}
        \end{subfigure}
            % \quad
        \begin{subfigure}[b]{0.24\textwidth}   
            \centering 
            \includegraphics[width=\textwidth]{images/LastFM/AMF_nDCG_Top10.png}
            \caption{\small \textbf{AMF}}
            \label{fig:testb}
        \end{subfigure}
        \begin{subfigure}[b]{0.24\textwidth}
            \centering
            \includegraphics[width=\textwidth]{images/LastFM/BPR-MF_ICov_Top10.png}
            \caption{\small  \textbf{BPR-MF}}
            \label{fig:testc}
        \end{subfigure}
            % \quad
        \begin{subfigure}[b]{0.24\textwidth}   
            \centering 
            \includegraphics[width=\textwidth]{images/LastFM/AMF_ICov_Top10.png}
            \caption{\small \textbf{AMF}} 
            \label{fig:testd}
        \end{subfigure}
        
                \vskip\baselineskip
        
        \begin{subfigure}[b]{0.24\textwidth}
            \centering
            \includegraphics[width=\textwidth]{images/ML1M/BPR-MF_nDCG_Top10.png}
            \caption{\small  \textbf{BPR-MF}}
            \label{fig:testa}
        \end{subfigure}
            % \quad
        \begin{subfigure}[b]{0.24\textwidth}   
            \centering 
            \includegraphics[width=\textwidth]{images/ML1M/AMF_nDCG_Top10.png}
            \caption{\small \textbf{AMF}}
            \label{fig:testb}
        \end{subfigure}
        \begin{subfigure}[b]{0.24\textwidth}
            \centering
            \includegraphics[width=\textwidth]{images/ML1M/BPR-MF_ICov_Top10.png}
            \caption{\small  \textbf{BPR-MF}}
            \label{fig:testc}
        \end{subfigure}
            % \quad
        \begin{subfigure}[b]{0.24\textwidth}   
            \centering 
            \includegraphics[width=\textwidth]{images/ML1M/AMF_ICov_Top10.png}
            \caption{\small \textbf{AMF}} 
            \label{fig:testd}
        \end{subfigure}
        \vskip\baselineskip
        \begin{subfigure}[b]{\textwidth}  
            \centering
            \includegraphics[width=0.75\textwidth]{images/legend_.png}
        \end{subfigure}
        
        
        \end{adjustbox}
        \caption{
        \felice{This figure can be a substitute of Figure 1 since here we have both datasets.}
        \lfm (first-row) and \ml (second-row) dataset results for an accuracy ($nDCG@10$) and diversity ($ICov@10$) metrics. First two figures of each row show the effects of adversarial attacks on the $nDCG@10$ on BPR-MF and AMF respectively. Last two figures report the variation of the $ICov@10$. Figures report also the results of the random recommender (violet dotted line).  Attacks produce recommendation performance with low-valued accuracy (close to the random RS) and diversity. So, in summary, attacks make the initial recommender worse than a random one.}
        \label{fig:testoverall_effect_full}
        
\end{figure}
\newpage

==> tables/dataset.tex <==
% \begin{table}[!h]
%     \centering
%     \caption{Dataset statistics. $|\mathcal{U}|$ is the number of the users, $|\mathcal{I}|$ is the number of items, and $|\mathcal{F}|$ is the number of recorded feedback.}
%     \begin{tabular}{l c c c c}
%         \toprule
%         \textbf{Dataset} & \multicolumn{1}{c}{$|\mathcal{U}|$} & \multicolumn{1}{c}{$|\mathcal{I}|$} & \multicolumn{1}{c}{$|\mathcal{F}|$} & \multicolumn{1}{c}{$\text{density}$} \\
%         \bottomrule
%         \multicolumn{1}{l }{\ml } & $ 6,040 $ & $ 3,706$ & $ 1,000,209 $ & $0.0447$ \\ 
%         \multicolumn{1}{l}{\lfm } & $ 2,847 $ & $ 33,164 $  & $ 935,875 $ & $0.0099 $ \\ 
%         \bottomrule
%     \end{tabular}
%     \label{table:dataset_statistics}
% \end{table}


\begin{table}[!h]
    \centering
    \caption{Dataset statistics. $|\mathcal{U}|$ is the number of the users, $|\mathcal{I}|$ is the number of items, and $|\mathcal{F}|$ is the number of recorded feedback.}
    \begin{tabular}{l c c c c}
        \toprule
        \textbf{Dataset} & \multicolumn{1}{c}{$|\mathcal{U}|$} & \multicolumn{1}{c}{$|\mathcal{I}|$} & \multicolumn{1}{c}{$|\mathcal{F}|$} \\
        \bottomrule
        \multicolumn{1}{l }{\ml } & $ 6,040 $ & $ 3,706$ & $ 1,000,209 $ \\ 
        \multicolumn{1}{l}{\lfm } & $ 2,847 $ & $ 33,164 $  & $ 935,875 $ \\ 
        \bottomrule
    \end{tabular}
    \label{table:dataset_statistics}
\end{table}

==> tables/stat-gorups.tex <==
\begin{table}[htbp]
\caption{\walter{@Alejandro: we have prepared and introduced this table. Do you think we need it? In case, where do we put it?}}
\small
\begin{tabular}{lrrrrrrrrrr}
\toprule
 & \multicolumn{ 4}{c}{Items Popularity} & \multicolumn{ 4}{c}{Users Interactions} & \multicolumn{ 2}{c}{Users Gender} \\ 
 & \multicolumn{1}{r}{c0} & c1 & c2 & c3 & \multicolumn{1}{r}{c0} & c1 & c2 & c3 & \multicolumn{1}{r}{c0} & c1 \\ \cmidrule (r){1-1}\cmidrule (rl){2-5}\cmidrule (rl){6-9}\cmidrule (rl){10-11}%
\lfm & 8508 & \multicolumn{1}{r}{8124} & \multicolumn{1}{r}{8443} & \multicolumn{1}{r}{8089} & 716 & \multicolumn{1}{r}{710} & \multicolumn{1}{r}{709} & \multicolumn{1}{r}{712} & 2037 & \multicolumn{1}{r}{353} \\ 
% & \multicolumn{1}{r}{457} \\ \hline
\ml & 945 & \multicolumn{1}{r}{908} & \multicolumn{1}{r}{927} & \multicolumn{1}{r}{926} & 1522 & \multicolumn{1}{r}{1516} & \multicolumn{1}{r}{1499} & \multicolumn{1}{r}{1503} & 4331 & \multicolumn{1}{r}{1709} \\ \bottomrule
% & NaN \\ \hline
\end{tabular}
\label{table:groups}
\end{table}


==> tables/table.lastfm.fair.tex <==
\begin {tabular}{rrrrrrr}%
\toprule && \multicolumn {5}{c}{User interactions} \\Model&&$f_0$&$f_1$&$f_4$&MADr&MADR\\\midrule %
\multirow {4}{*}{\noDef }&initial&\pgfutilensuremath {-0.014}&\pgfutilensuremath {-0.815}&$\bf \pgfutilensuremath {-0.352}$&$\bf \pgfutilensuremath {0.557}$&\pgfutilensuremath {0.051}\\%
&FGSM&$\bf \pgfutilensuremath {-0.007}$&\pgfutilensuremath {-0.723}&\pgfutilensuremath {-0.395}&\pgfutilensuremath {0.686}&\pgfutilensuremath {0.022}\\%
&BIM&\pgfutilensuremath {-0.207}&$\bf \pgfutilensuremath {-0.240}$&\pgfutilensuremath {-2.596}&\pgfutilensuremath {3.153}&\pgfutilensuremath {0.005}\\%
&PGD&\pgfutilensuremath {-0.026}&\pgfutilensuremath {-0.278}&\pgfutilensuremath {-0.694}&\pgfutilensuremath {3.062}&$\bf \pgfutilensuremath {0.002}$\\%
\midrule \multirow {4}{*}{\Def }&initial&$\bf \pgfutilensuremath {-0.026}$&$\bf \pgfutilensuremath {-0.912}$&\pgfutilensuremath {-0.290}&\pgfutilensuremath {2.057}&\pgfutilensuremath {0.079}\\%
&FGSM&\pgfutilensuremath {-0.028}&\pgfutilensuremath {-0.922}&\pgfutilensuremath {-0.279}&$\bf \pgfutilensuremath {1.060}$&\pgfutilensuremath {0.074}\\%
&BIM&\pgfutilensuremath {-0.066}&\pgfutilensuremath {-1.246}&$\bf \pgfutilensuremath {-0.199}$&\pgfutilensuremath {6.127}&\pgfutilensuremath {0.046}\\%
&PGD&\pgfutilensuremath {-0.063}&\pgfutilensuremath {-1.226}&\pgfutilensuremath {-0.209}&\pgfutilensuremath {7.015}&$\bf \pgfutilensuremath {0.046}$\\\bottomrule %
\end {tabular}%


==> tables/table.ml.fair.tex <==
\begin {tabular}{rrrrrrrrrrrr}%
\toprule &&\multicolumn {5}{c}{User gender} & \multicolumn {5}{c}{User interactions} \\Model&&$f_0$&$f_1$&$f_2$&MADr&MADR&$f_0$&$f_1$&$f_4$&MADr&MADR\\\midrule %
\multirow {4}{*}{\noDef }&initial&\pgfutilensuremath {-0.135}&\pgfutilensuremath {-0.001}&\pgfutilensuremath {-0.587}&$\bf \pgfutilensuremath {0.050}$&\pgfutilensuremath {0.003}&\pgfutilensuremath {-0.119}&$\bf \pgfutilensuremath {-0.135}$&\pgfutilensuremath {-1.495}&\pgfutilensuremath {0.618}&\pgfutilensuremath {0.030}\\%
&FGSM&$\bf \pgfutilensuremath {-0.132}$&\pgfutilensuremath {-0.001}&$\bf \pgfutilensuremath {-0.579}$&\pgfutilensuremath {0.067}&\pgfutilensuremath {0.002}&\pgfutilensuremath {-0.113}&\pgfutilensuremath {-0.156}&\pgfutilensuremath {-1.529}&$\bf \pgfutilensuremath {0.614}$&\pgfutilensuremath {0.028}\\%
&BIM&\pgfutilensuremath {-0.165}&$\bf \pgfutilensuremath {0.000}$&\pgfutilensuremath {-0.662}&\pgfutilensuremath {0.373}&\pgfutilensuremath {0.003}&$\bf \pgfutilensuremath {-0.004}$&\pgfutilensuremath {-0.534}&$\bf \pgfutilensuremath {-0.685}$&\pgfutilensuremath {1.781}&$\bf \pgfutilensuremath {0.002}$\\%
&PGD&\pgfutilensuremath {-0.132}&\pgfutilensuremath {-0.001}&\pgfutilensuremath {-0.579}&\pgfutilensuremath {0.234}&$\bf \pgfutilensuremath {0.001}$&\pgfutilensuremath {-0.025}&\pgfutilensuremath {-0.318}&\pgfutilensuremath {-0.918}&\pgfutilensuremath {1.564}&\pgfutilensuremath {0.005}\\%
\midrule \multirow {4}{*}{\Def }&initial&\pgfutilensuremath {-0.141}&\pgfutilensuremath {-0.001}&\pgfutilensuremath {-0.603}&\pgfutilensuremath {0.084}&\pgfutilensuremath {0.004}&\pgfutilensuremath {-0.094}&$\bf \pgfutilensuremath {-0.159}$&\pgfutilensuremath {-1.342}&\pgfutilensuremath {1.995}&\pgfutilensuremath {0.028}\\%
&FGSM&$\bf \pgfutilensuremath {-0.140}$&\pgfutilensuremath {-0.001}&$\bf \pgfutilensuremath {-0.599}$&$\bf \pgfutilensuremath {0.038}$&$\bf \pgfutilensuremath {0.004}$&\pgfutilensuremath {-0.095}&\pgfutilensuremath {-0.163}&\pgfutilensuremath {-1.416}&$\bf \pgfutilensuremath {1.674}$&\pgfutilensuremath {0.025}\\%
&BIM&\pgfutilensuremath {-0.190}&$\bf \pgfutilensuremath {0.000}$&\pgfutilensuremath {-0.724}&\pgfutilensuremath {0.302}&\pgfutilensuremath {0.005}&\pgfutilensuremath {-0.014}&\pgfutilensuremath {-0.428}&\pgfutilensuremath {-0.724}&\pgfutilensuremath {4.175}&\pgfutilensuremath {0.005}\\%
&PGD&\pgfutilensuremath {-0.212}&\pgfutilensuremath {-0.002}&\pgfutilensuremath {-0.777}&\pgfutilensuremath {0.328}&\pgfutilensuremath {0.006}&$\bf \pgfutilensuremath {-0.010}$&\pgfutilensuremath {-0.420}&$\bf \pgfutilensuremath {-0.707}$&\pgfutilensuremath {4.177}&$\bf \pgfutilensuremath {0.004}$\\\bottomrule %
\end {tabular}%

